Data-driven modeling and control of large-scale dynamical systems in the Loewner framework

In this contribution, we discuss the modeling and model reduction framework known as the Loewner framework. This is a data-driven approach, applicable to large-scale systems, which was originally developed for applications to linear time-invariant systems. In recent years, this method has been extended to a number of additional more complex scenarios, including linear parametric or nonlinear dynamical systems. We will provide here an overview of the latter two, together with time-domain extensions. Additionally, the application of the Loewner framework is illustrated by a collection of practical test cases. Firstly, for data-driven complexity reduction of the underlying model, and secondly, for dealing with control applications of complex systems (in particular, with feedback controller design).

==> figures/controlLoopInitial.tex <==
\tikzstyle{block} = [draw, thick,fill=blue!20, rectangle, minimum height=4em, minimum width=6em,rounded corners]
\tikzstyle{sum} = [draw, thick,fill=blue!20, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thick,black}]
\tikzstyle{connector} = [->,thick]

% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=3cm,>=latex']
    % We start by placing the blocks
    \node [input, name=input] {};
    \node [sum, right of=input] (sum) {};
    \node [block, right of=sum] (controller) {$\mathbf K(s)$};
    %\node [block, right of=controller, pin={[pinstyle]above:Disturbances},node distance=3cm] (system) {System};
    \node [block, right of=controller, node distance=4cm] (system) {$\Htran_{x_m}(s)$};
    %\node [block, right of=controller, node distance=3cm] (reference) {$M$};
    % We draw an edge between the controller and system block to 
    % calculate the coordinate u. We need it to place the measurement block. 
    \draw [connector] (controller) -- node[name=u] {$\red{\u}$} (system);
    \node [output, right of=system] (output) {};
    %\node [block, below of=u] (measurements) {Measurements};

    % Once the nodes are placed, connecting them is easy. 
    \draw [connector] (input) -- node {$\green{\mathbf r}$} (sum);
    \draw [connector] (sum) -- node {$\mathbf e$} (controller);
    \draw [connector] (system) -- node [name=y] {$\red{\y}$}(output);
    %\draw [->] (y) |-| (measurements);
    %\draw [->] (measurements) -| node[pos=0.99] {$-$} node [near end] {$y_m$} (sum);
    \draw [connector] (output)+(-0.3cm,0) -- ++(-0.3cm,-1.5cm) -| node [near start] {} (sum.south);
    
%    \pause
%    \node [block, above of=u, node distance=1cm,green!30,text=black,thick,draw=black,rounded corners] (model) {Reference model};
%    \draw [connector,green!30] (output)+(-0.3cm,0) |- node [near start] {} (model.east);
%    \draw [-,thick,green!30] (model.west) -| node [near start] {} (input);
    
\end{tikzpicture}

==> temp.tex <==
\subsection{Victor damping}

In this particular case, the parameter is the damping coefficient $c_d$. Our objective is to come up with a parametrized linear model that is able to faithfully reproduce the original transfer function on a particular range of frequencies as well as on a target  parameter range. As before we take measurements and we decide what order should we choose for the reduced model by inspecting the singular value decay. The frequency 'interest' range was chosen as for the other experiments, while the parameter 'target range' was taken to be $[10^{-5},10^{7}]$. For 30 values of $c_d$ in this range, we evaluate the transfer function $H_{orig}$ at 100 sampling points.

\begin{figure}[h] \label{fig11} \vspace{-3mm}
	\begin{center}
		\includegraphics[scale=0.28]{figures/Beam/plot_beam16.eps}
		\vspace{-3mm}
		\caption{Singular values decay}
	\end{center} \vspace{-6mm}
\end{figure}

The plot above depicts two types of singular values. On one hand, we form Loewner matrices by using measurements for varying frequency and constant parameter ( marked with green). On the other hand, we form Loewner matrices by using measurements for varying parameter and constant frequency ( marked with blue).

By investigating the drop in the SV plot, we decide to use reduction orders $r_s = 30$ and $r_p = 14$ for building the two dimensional Loewner matrix. Then construct a reduced linear parametric model which is sampled on the same frequency and parameter range as before. When comparing to the original samples, the overall result is satisfactory:




%%%%%%%%%%%%% PK limitations
The closed-loop performances are limited by the system's right hand side poles $\{p_j\}_{j=1}^{n_p}$ and zeros $\{z_i\}_{i=1}^{n_z}$ (and their respective output directions in the MIMO case) defined as $\Htran_{x_m}(z_i) = 0$ and $\Htran_{x_m}(p_j) = \infty$. Finally, the class $\mathcal{M}$ of achievable reference models is defined as follows: 
\begin{equation}
\mathcal{M}=\big\{\mathbf{M}\in \mathcal{H}_\infty : \, \mathbf{M}(z_i) = 0 \text{ and } \mathbf{M}(p_j) = 1\big\}.
\end{equation}


In the general case, the right half plane poles and zeros of the system are estimated in \cite{kergus2019} in order to build an achievable reference model on the basis of the initial specifications given by the user. This is made possible through a data-driven stability analysis introduced in \cite{cooman2018model} and the associated estimation of instabilities presented in \cite{cooman2018estimating}. 

Here, the PDE describing the system's dynamic is known and allows to determine the performance limitations without applying the aforementioned data-driven stability analysis. The instabilities are $\Htran_{x_m}(+\infty)=0$ and $\Htran_{x_m}(0)=\infty$, implying that the reference model should satisfy $\mathbf{M}(+\infty)=0$ and $\mathbf{M}(0)=1$.

As shown in \cite{kergus2019appendix}, once the set $\mathcal{M}$ of achievable reference models is determined, the one chosen in this set influences a lot the control design. To illustrate this point, the \textbf{L-DDC} algorithm is applied on the proposed example using two reference models $\mathbf{M}_1$ and $\mathbf{M}_2$. $\mathbf{M}_1$ is chosen as a perfectly damped second-order model with a natural frequency $\omega_0=0.5\textnormal{ rad.s}^{-1}$ and reads
$$
\mathbf{M}_1(s)=\frac{1}{s^2/\omega_0^2+2s/\omega_0+1},
$$
satisfying the performance limitations of the system. The second reference model $\mathbf{M}_2$ is the closed-loop obtained in the model-based control design obtained in Section \ref{sec-model-based} ($\mathbf{M}_2=\hat{\mathbf{M}}$, see Figure \ref{fig:M})\footnote{Since the procedure used to get $\hat{\mathbf{M}}$ preserves internal stability, the obtained closed-loop is necessarily achievable by the plant $\Htran_{x_m}$.}. 


%%%%%%%%%%% Stability data 
One of the major challenges in this data-driven control strategy is to preserve internal stability. While the ideal controller is known to be stabilising thanks to the choice of an achievable reference model, see \cite{kergus2019}, there is no guarantee regarding the reduced-order controllers. Therefore, it is necessary to analyse the internal stability during the controller reduction step. To that extent, the resulting closed-loop is written as on Figure \ref{fig:small_gain}. This scheme makes the controller error appear as a perturbation. 
\begin{figure}[h]
%\sidecaption
%\scalebox{.78}{\input{./figures/tikz/DDC/small_gain}}
\caption{Stability analysis of the closed-loop obtained with a reduced-order controller $\mathbf{K}$: the closed-loop is reformulated according to the controller modelling error $\mathbf{K}-\mathbf{K}^\star$.}
\label{fig:small_gain}
\end{figure}

It is then possible to apply the small-gain theorem: the interconnected system shown on Figure \ref{fig:small_gain} is well-posed and internally stable for all stable $\mathbf{\Delta}=\mathbf{K}-\mathbf{K}^\star$ with $\left\Vert \mathbf{\Delta} \right\Vert_\infty < \frac{1}{\gamma}$ if and only if $\left\Vert \Htran_{x_m}(1-\mathbf{M}) \right\Vert_\infty \leq\gamma$. The bound $\gamma$ on the controller modelling error can then be estimated using the data only as:
\begin{equation}
    \Tilde{\gamma}=\underset{i=1\dots m}{\textnormal{max}}\left| \Htran_{x_m}(\imath\omega_i)(1-\mathbf{M}(\imath\omega_i))\right|.
    \label{estimation_gamma}
\end{equation}
The evolution of the controller modelling error $\left\Vert \mathbf{K}-\mathbf{K}^\star \right\Vert_\infty$ according to the order of the reduced controller $\mathbf{K}$ is represented on Figure \ref{fig:reduction_K} for the two considered reference models, $\mathbf{M}_1$ and $\mathbf{M}_2$. According to Figure \ref{fig:reduction_K}, to ensure that the resulting closed-loop is internally stable, one may reduce $\mathbf{K}_1^\star$ up to $r=13$ and $\mathbf{K}_2^\star$ up to $r=2$.
\begin{figure}[h]
%\sidecaption
\centering
%\includegraphics[width=0.9\textwidth]{./figures/tikz/DDC/test_stabilite.pdf}
\caption{Evolution of the controller modelling error as a function of the controller reduction step.}
\label{fig:reduction_K}
\end{figure}

However, this stability test is too conservative: it is not possible to conclude anything regarding internal stability for controllers $\mathbf{K}$ for which $\left\Vert \mathbf{K}-\mathbf{K}^\star \right\Vert_\infty>\Tilde{\gamma}$. In the present case, both order one controllers given in \eqref{LDDC_controllers} stabilise internally the rational model. Another solution would be to use the model-free stability analysis presented in \cite{cooman2018model} but it may be complicated for the user to conclude regarding internal stability. To that extent, another approach to analyse stability in a data-driven framework is introduced in Section \ref{sec:stab}. 

